Deep Diving into BitTorrent Locality

A substantial amount of work has recently gone into localizing BitTorrent traffic within an ISP in order to avoid excessive and often times unnecessary transit costs. Several architectures and systems have been proposed and the initial results from specific ISPs and a few torrents have been encouraging. In this work we attempt to deepen and scale our understanding of locality and its potential. Looking at specific ISPs, we consider tens of thousands of concurrent torrents, and thus capture ISP-wide implications that cannot be appreciated by looking at only a handful of torrents. Secondly, we go beyond individual case studies and present results for the top 100 ISPs in terms of number of users represented in our dataset of up to 40K torrents involving more than 3.9M concurrent peers and more than 20M in the course of a day spread in 11K ASes. We develop scalable methodologies that permit us to process this huge dataset and answer questions such as: "\emph{what is the minimum and the maximum transit traffic reduction across hundreds of ISPs?}", "\emph{what are the win-win boundaries for ISPs and their users?}", "\emph{what is the maximum amount of transit traffic that can be localized without requiring fine-grained control of inter-AS overlay connections?}", "\emph{what is the impact to transit traffic from upgrades of residential broadband speeds?}".

==> otherpercentiles.tex <==


\section{Additional details on degradation of QoS}\label{app:otherpercentiles}

In Table~\ref{tab:40k-qos} we reported the degradation of QoS in terms of median download rate under the different policies for the six largest ISPs. In this section, we focus on the two largest ones, US1, EU1, and we compare the QoS degradation in terms of additional percentiles (5\%, 25\%, 50\%, 75\%, 95\%). Looking at Table~\ref{tab:otherpercentiles} we see that the reduction in terms of median is not much different than the reduction in terms of all other, but the two extreme, percentiles. The biggest difference is observed under Strict and is due to the heavy penalty paid by users downloading unlocalizable torrents, as explained in~Sect.~\ref{subsubsec:unlocalizable}. Notice that all observed difference are due to speed differences between ISP. Differences between access speed within the same ISP do not play a role here since under Ookla all clients of an ISP are assigned their country speed.

\begin{table}[htb]
{\small
\begin{center}
\begin{tabular}{l|l|l|l|l|l|}
ISP       & Prct 5   & Prct 25  & Prct 50 & Prct 75 & Prct 95 \\\hline
US1 (LOIF)&  -3.98\% & -7.93\%  & -6.71\% & -5.61\% & -5.87\% \\
EU1 (LOIF)&   1.53\% & -2.01\%  & -1.47\% & -2.51\% & -2.50\\
US1 (Locality)&-2.45\% &-3.38\% & -1.32\% &  1.20\% & 3.46\% \\
EU1 (Locality)& 3.83\% & 6.36\% &  3.33\% &  2.72\% & 6.69\% \\
US1 (Strict)&   24.87\% &-1.74\%&  2.88\% &  6.81\% &  16.81\% \\
EU1 (Strict)&   76.73\% & 16.07\% & 18.59\% & 18.00\% & 29.04\% \\
\end{tabular}
\end{center}}
\caption{QoS Degradation under {\tt mn40K} and Ookla speeds.} 
\label{tab:otherpercentiles} \end{table}


==> stability.tex <==
\subsection{Stability of results across datasets}

Next we look at how using different demographic and speed datasets affects our results.

\subsubsection{PirateBay's most popular torrents}

In Table~\ref{tab:top600-tt} we recompute the transit traffic savings compared to Random based the dataset {\tt pb600} of the 600 most popular torrents of PirateBay. In this case the savings are even higher. There are two reasons for this. First, Locality and LOIF have more internal nodes to use. Second, Random is impacted negatively because despite the increase in absolute number of locals, their relative percentage compared to the entire population shrinks.

\subsubsection{iPlane speeds}

In Table~\ref{tab:40k-tt-iplane} we return to the transit traffic
reductions under {\tt mn40K} but this time we compute them based
on iPlane~\cite{iplane_osdi} speeds. From
this dataset we can obtain for each ISP a distribution of speeds
for different clients as opposed to just the median value that we get
from Ookla~\cite{Stanford:page}. However iPlane has fewer
measurements than the commercial service and thus we use it for
validation instead of as our main speed dataset. Comparing
Table~\ref{tab:40k-tt-iplane} with Table~\ref{tab:40k-tt} we see
that the results from the two speed datasets are in good agreement
for all overlay policies except LOIF. In LOIF, speed affects
the construction of the overlay and thus any speed disagreement
between the two datasets impacts more heavily the produced transit
savings. In Fig.~\ref{fig:cdf_country_speed} we computed the
median country speed from iPlane and plotted it next to the
corresponding one from Ookla. One can see that there is some
discrepancy between the two and this justifies the
differences seen in the produced results for LOIF.

\subsection{Stability of results across time}

Next we evaluate the effect of time on our obtained transit
savings. We look at hourly and weekly time scales.

\subsubsection{Hours}

Torrent membership is dynamic and thus if examined at different
hours of the day a torrent will have different participants. In
this section we evaluate the impact of dynamic membership on our
results. We do so using {\tt pb600}. Since we can crawl
this dataset in less than an hour, we performed 24 crawls of
it across the different hours of a day. In Fig.~\ref{fig:periodic}
we plot the resulting transit savings for ISP US1 at different
hours. One can see that dynamic membership has a very small impact
on the calculated transit savings. Since {\tt pb600} is biased
towards large torrents, we wanted to evaluate also an unbiased
dataset and for this purpose we used {\tt mn3K}. Again, Fig.~\ref{fig:periodic}
shows that our computations are quite stable. 

The depicted stability should not come as a surprise. First,
transit traffic reduction is a relative metric so it is less
sensitive to diurnal variations of torrent population than, \eg,
the absolute amount of transit traffic. Second, the aggregation
effect from multiple independent torrents naturally smooths out
any variability at specific hours.

\begin{figure}[tb]
\flushleft
\includegraphics[width=3.7in]{figures/stability2}
\caption{Transit traffic reduction for US1 during different times of a day under Ookla speeds.}
\label{fig:periodic}
\end{figure}

\subsubsection{Weeks}

Next we recompute the transit savings for all 6 ISPs on different
days. We do so by using 3 snapshots of {\tt mn40K} taken from 3
consecutive weeks. In each case the dataset contains the 40K
\emph{latest} Mininova torrents and thus apart from membership
differences on the same torrent, the snapshots also differ in
terms of included torrents: the second one, \eg, contains the new
torrents of the latest week, which are not included in the
previous one. The transit savings differ by less than 7\% in all
cases.

